Learning to Learn without Gradient Descent by Gradient Descent

We learn recurrent neural network optimizers trained on simple synthetic functions by gradient descent. We show that these learned optimizers exhibit a remarkable degree of transfer in that they can be used to efficiently optimize a broad range of derivative-free black-box functions, including Gaussian process bandits, simple control objectives, global optimization benchmarks and hyper-parameter tuning tasks. Up to the training horizon, the learned optimizers learn to trade-off exploration and exploitation, and compare favourably with heavily engineered Bayesian optimization packages for hyper-parameter tuning.

==> includes/related_work.tex <==
\section{Comparison Between DNC and LSTM Core}

We show the comparison of our neural network optimizers with a DNC core and an LSTM core on the random functions sampled from the training distribution in Figure \ref{fig:gp_core}.

\begin{figure*}[tb]%
\centering
\includegraphics[width=\textwidth]{figs/GPSample_core}
\caption{Average test loss with $95\%$ confidence interval on functions sampled from the GP prior.}
\label{fig:gp_core}
\end{figure*}

